A Survey on Computational Pathology Foundation Models: Datasets, Adaptation Strategies, and Evaluation Tasks

Computational pathology foundation models (CPathFMs) have emerged as a powerful approach for analyzing histopathological data, leveraging self-supervised learning to extract robust feature representations from unlabeled whole-slide images. These models, categorized into uni-modal and multi-modal frameworks, have demonstrated promise in automating complex pathology tasks such as segmentation, classification, and biomarker discovery. However, the development of CPathFMs presents significant challenges, such as limited data accessibility, high variability across datasets, the necessity for domain-specific adaptation, and the lack of standardized evaluation benchmarks. This survey provides a comprehensive review of CPathFMs in computational pathology, focusing on datasets, adaptation strategies, and evaluation tasks. We analyze key techniques, such as contrastive learning and multi-modal integration, and highlight existing gaps in current research. Finally, we explore future directions from four perspectives for advancing CPathFMs. This survey serves as a valuable resource for researchers, clinicians, and AI practitioners, guiding the advancement of CPathFMs toward robust and clinically applicable AI-driven pathology solutions.

==> sections/methods_old.tex <==
\begin{table*}[ht]
\centering
\begin{threeparttable}
\begin{tabular}{ccccc}
\toprule
% \textbf{} & \textbf{Method} & \textbf{SSL Framework} & \textbf{Visual (\& Language) Backbone [\# Param.]}  & \textbf{Image Type}\tnote{$\dagger$} \\
% 这里先只写visual的backbone吧，有些text的不是很确定。。。
\textbf{} & \textbf{Methods} & \textbf{SSL Framework} & \textbf{Visual Backbone [\# Param.]}  & \textbf{\textcolor{red}{Image Type}}\tnote{$\dagger$} \\ \midrule
\multirow{12}{*}{\makecell[c]{\rotatebox{90}{\textbf{Uni-modal}}}} & CTransPath \cite{CTransPath} & MoCo v3 & Swin Transformer [28M] & T \\ 
    & REMEDIS \cite{REMEDIS} & SimCLR  &  ResNet-152 (2$\times$) [232M] & T \\
    & Lunit DINO \cite{Lunit} & DINO  & ViT-S/(8,16)\tnote{$\ddagger$}\;\;[22M] & T \\
    & Phikon \cite{Phikon} & iBOT & ViT-B/16 [86M] & T \\
    
    & Virchow \cite{Virchow} & DINOv2 & ViT-H/14 [632M] & T  \\
    & \multirow{2}{*}{Campanella et al.\cite{campanella2024computational}} & DINO & ViT-S [22M], ViT-B [86M] & \multirow{2}{*}{T}  \\
    &  & MAE & ViT-L [307M] & \\
    & RudolfV \cite{RudolfV} & DINOv2 & ViT-L/14 [307M] & T  \\
    & \multirow{2}{*}{Kaiko\cite{Kaiko}} & DINO & ViT-S/(8,16) [22M], ViT-B/(8,16) [86M] & \multirow{2}{*}{T}  \\
    &   & DINOv2 & ViT-L/14 [307M]&   \\
    & GigaPath \cite{GigaPath} & DINOv2 & ViT-G/14 [1.1B] + LongNet [125M]& S \\
    & Hibou \cite{Hibou} & DINOv2 & ViT-B/14 [86M], ViT-L/14 [307M]& T \\
    & Virchow2 \cite{Virchow2} & DINO & ViT-B/16 [86M] & T \\ 
    & Phikon-v2 \cite{Phikon-v2} & DINOv2 & ViT-L/16 [307M] & T \\

    & UNI \cite{UNI} & DINOv2 & ViT-L/16 [307M] & T  \\ \midrule
    
% \multirow{4}{*}{\makecell[c]{\rotatebox{90}{\textbf{Multi-modal}}}} & PLIP \cite{PLIP} & CLIP & ViT-B/32 [86M] \& \textcolor{red}{CLIP Text Encoder [76M]} & T  \\
%     & CONCH \cite{CONCH} & CoCa & ViT-B/16 [86M] \& 12 Transformer Layers (2$\times$)  [14M] & T \\
%     & PRISM \cite{PRISM} & CoCa & ViT-H/14 [632M] + Perceiver [105M] \& BioGPT [345M] & S \\ 
    
%     & PathChat \cite{PathChat} & DINOv2, CoCa & 1 & T \\ 
%     & CHIEF \cite{CHIEF} & CLIP & Swin Transformer [28M] \& CLIP Text Encoder [76M]  & S \\ 

\multirow{4}{*}{\makecell[c]{\rotatebox{90}{\textbf{Multi-modal}}}} & PLIP \cite{PLIP} & CLIP & ViT-B/32 [86M] & T  \\
    & PathCLIP \cite{PathCLIP}& CLIP &  ViT-B/32 [86M] & T \\
    % PathAsst借助PathCLIP作为visual component，然后通过两个阶段进行训练，第一个阶段通过180K instruction-following 来训练PathCLIP和LLM之间的FC layer以align the vision encoder with the LLM。第二个阶段用具有更长token的指令集微调LLM。其中用了很多instruction-following data tailored for model invocation来让PathAsst能够调用一些specialized pathological models
    & PathAsst \cite{PathCLIP} & CLIP & PathCLIP [86M] & T \\
    & CONCH \cite{CONCH} & CoCa & ViT-B/16 [86M] & T \\
    & PRISM \cite{PRISM} & CoCa & Virchow [632M] + Perceiver [105M] & S \\ 
    & CHIEF \cite{CHIEF} & CLIP & CTransPath [28M] & S \\
    & PathChat \cite{PathChat} & DINOv2, CoCa & UNI [307M] & T \\ 
    
    & TITAN \cite{TITAN} & iBOT, CoCa &  ViT-S [22M] & S \\ \bottomrule
\end{tabular}
\begin{tablenotes}
    % \item[$\dagger$] The abbreviations stand for uni-modal (U) and multi-modal (M).
    \item[$\dagger$] The abbreviations stand for tile-level (T) and slide-level (S).
    \item[$\ddagger$] “/$n$” denotes a patch size of $n\times n$ pixels; “/$(n,m)$” denotes “/$n$” and “/$m$” two models.
    \end{tablenotes}
\end{threeparttable}
\caption{Sample Table - methods categorized by Tile-level and Slide-level}
\label{tab:methods}
\end{table*}

\begin{table*}[ht]
\centering
\begin{threeparttable}
\begin{tabular}{ccccccccc}
\toprule
\textbf{Method} & \textbf{\# WSIs} & \textbf{\# Tiles} & \textbf{Tile Size} & \textbf{FoV} & \textbf{Staining Type} & \textbf{Source} \\ \midrule

 CTransPath & 32.2K & 15.6M & $\text{1024}^{\text{2}}$ & 20$\times$ & H\&E & TCGA, PAIP \\ 
REMEDIS & 29.0K & 50.0M & $\text{224}^{\text{2}}$ & 20$\times$ & H\&E & TCGA, JFT54* (natural) \\ 
Lunit DINO & 36.7K & 32.6M & $\text{512}^{\text{2}}$ & \{20, 40\}$\times$ & H\&E (with Aug.) & TCGA, TULIP* \\ 
Phikon &6.1K & 43.4M & $\text{224}^{\text{2}}$ & 20$\times$ & H\&E & TCGA \\ 

Virchow  & 1.5M & 2.0B & $\text{224}^{\text{2}}$ & 20$\times$ & H\&E & MSKCC*  \\ 

% UNI & U & 100K & 100M & 256$\times$256, 512$\times$512 & 20$\times$ & H\&E &  MGH*, BWH*, GTEx  \\ 
UNI & 100K & 100M & $\text{256}^{\text{2}}$, $\text{512}^{\text{2}}$ & 20$\times$ & H\&E &  MGH*, BWH*, GTEx  \\ 

Campanella et al.  & 423K & 1.6B, 3.2B & $\text{224}^{\text{2}}$ & 20$\times$ & H\&E & MSHS* \\ 
    RudolfV & 134K & 1.2B &  $\text{256}^{\text{2}}$ & \{20, 40, 80\}$\times$ & H\&E, IHC, other & TCGA, \textit{Proprietary}*   \\ 
Kaiko & 29.0K & 256M &  $\text{256}^{\text{2}}$ & \{5, 10, 20, 40\}$\times$ & H\&E & TCGA  \\ 
GigaPath & 171K & 1.4B &  $\text{256}^{\text{2}}$ & 20$\times$ & H\&E, IHC &   PHS*\\ 
Hibou & 1.1M & 512M, 1.2B &  $\text{224}^{\text{2}}$ & 20$\times$ & H\&E, non-H\&E &  \textit{Proprietary}*\\ 
Virchow2 & 3.1M & 2.0B &  $\text{392}^{\text{2}}$ & \{5, 10, 20, 40\}$\times$ & H\&E, IHC & extended MSKCC*\\ 
Phikon-v2 & 58.0K & 456M & $\text{224}^{\text{2}}$ & 20$\times$ & various & TCGA, CPTAC, GTEx, etc. \\ 


\bottomrule
\end{tabular}
\begin{tablenotes}
    \item[$\ast$] Internally collected dataset.
    \end{tablenotes}
\end{threeparttable}

\caption{Pre-training datasets for uni-modal methods}
\label{tab:pretrain-datasets-uni}

\end{table*}

% \begin{table*}[ht]
% \centering
% \begin{threeparttable}
% \begin{tabular}{cccccccc}
% \toprule
% \textbf{Method} & \textbf{\# Slide-Report}\tnote{$\dagger$} & \textbf{\# Tile-Caption} & \textbf{Tile Size} & \textbf{FoV} & \textbf{Staining Type} & \textbf{Source} \\ \midrule


% PLIP & - & 208K & $\text{224}^{\text{2}}$ & Various & \textcolor{red}{H\&E} & Twitter, PathLAION \\ 
% PRISM & 587K-195K & - & $\text{224}^{\text{2}}$ & 20$\times$ & H\&E & TCGA, \textit{Proprietary}* \\ 

% PathChat & - &  & $\times$ &  &  & \\ 

% CHIEF &  &  & $\text{256}^{\text{2}}$ & 10$\times$ &  & \\ 


% % remember the source dataset citation


% \bottomrule
% \end{tabular}
% \begin{tablenotes}
%     \item[$\dagger$] Note that one or more WSIs usually have a corresponding clinical report in practice.
%     \item[$\ast$] Internally collected dataset.
%     \end{tablenotes}
% \end{threeparttable}

% \caption{Pre-training datasets for multi-modal methods}
% \label{tab:pretrain-datasets-multi}
% \end{table*}

\begin{table*}[ht]
\centering
\begin{threeparttable}
\begin{tabular}{ccccc}
\toprule
\textbf{Method} & \textbf{Statistical Description}\tnote{$\dagger$}  & \textbf{Staining Type} & \textbf{Source} \\ \midrule


PLIP &  208K tile-caption pairs & \textcolor{red}{H\&E} & Twitter, PathLAION \\ 
PathCLIP &  207K tile-caption pairs & H\&E, IHC & PubMed, LBC* \\ 
PathAsst &  180K; 35K instruction-following pairs & H\&E, IHC & PubMed, LBC*  \\ 
CONCH & 1.17M tile-caption pairs & H\&E, IHC, special & PMC OA, EDU*\\ 
PRISM & 587K WSIs + 195K clinical reports\tnote{$\ddagger$} & H\&E & TCGA, \textit{Proprietary}* \\ 

CHIEF & 15.6M tiles; 60K WSIs-anatomical sites pairs & H\&E & TCGA, \textit{Proprietary}*, etc.\\ 

PathChat & \makecell[c]{100M tiles; 1.2M tile-caption pairs; 467K instructions}    & H\&E, IHC & \makecell[c]{PubMed, TCGA, \textit{Proprietary}*}\\ 

TITAN & 336K WSIs; 423K tile-caption pairs; 183K WSI-report pairs & H\&E, IHC & TCGA, \textit{Proprietary}*, etc.\\ 


% remember the source dataset citation


\bottomrule
\end{tabular}
\begin{tablenotes}
    \item[$\dagger$] Multimodal foundation models are typically trained in several stages, with different stages of data separated by semicolons (";").
    \item[$\ddagger$] Note that one or more WSIs usually have a corresponding clinical report in practice.
    \item[$\ast$] Internally collected dataset.
    \end{tablenotes}
\end{threeparttable}

\caption{Pre-training datasets for multi-modal methods.}
\label{tab:pretrain-datasets-multi}
\end{table*}

\subsection{Uni-Modal}

Summary
% 蓝色部分可能能统一提出来一章介绍相关的SSL framework

\textbf{CTransPath} \cite{CTransPath}
aims to develop a histopathology-oriented contrastive learning (CL) approach. It introduces the SRCL framework, which is pre-trained on a dataset consisting of 15.6 million tiles cropped from over 30,000 whole-slide images (WSIs). The framework adds a branch to MoCo v3 \cite{MoCo3} to generate queries that retrieve semantically similar samples from the memory bank as positive samples, thus guiding the network's training with a semantically relevant contrastive loss. It employs a hybrid architecture of CNN and Swin Transformer \cite{Swin} as the backbone to simultaneously capture both local and global information.

\textbf{REMEDIS} \cite{REMEDIS}, as a unified representation-learning strategy, pretrains ResNet-152 \cite{resnet} in two stages. First, it undergoes large-scale supervised pretraining on natural images, followed by transfer to a self-supervised learning algorithm based on contrastive learning (SimCLR) \cite{SimCLR} for contrastive self-supervised learning. It improves both in-distribution (ID) and out-of-distribution (OOD) performance across multiple medical imaging tasks.

\textit{Kang et al.}~\cite{Lunit} adapt SSL for pathology within four SSL framework by introducing data augmentation techniques such as random vertical flips and stain augmentations, as well as a data curation technique utilizing multiple fields of view (FoVs). Their method under the DINO framework \cite{DINO} is referred to as \textbf{Lunit DINO}, which trains ViT-S \cite{ViT-S} on 32.6 million image tiles with 20$\times$ (0.5$\mu$m/px) and 40$\times$ (0.25$\mu$m/px) objective magnification. Their study demonstrates that large-scale domain-aligned pre-training is beneficial for pathology. 

% \textbf{Phikon}\footnote{The authors state that they built the best model using the largest and most diverse dataset on ViT-B/16. Therefore, Phikon typically refers to the model trained on 43.4 million tiles using ViT-B/16.} \cite{Phikon} trains a ViT within the iBOT framework \cite{iBOT} using Masked Image Modeling (MIM), \textcolor{blue}{which randomly applies masks to certain regions and reconstructs the masked areas to learn valuable and meaningful representations for a given image tile}. They focuse on investigating the scalability of the iBOT framework in pathology across three aspects: the scale of the backbone (ViT-S, ViT-B and ViT-L), the size of the pre-training dataset (4.4M and 43.4M tiles), and its diversity (colon-specific and pan-cancer).

\textit{Filiot et al.}~\cite{Phikon} train a ViT within the iBOT framework \cite{iBOT} using Masked Image Modeling (MIM), which randomly applies masks to certain regions and reconstructs the masked areas to learn valuable and meaningful representations for a given image tile. They focuse on investigating the scalability of the iBOT framework in pathology across three aspects: the scale of the backbone (ViT-S, ViT-B and ViT-L), the size of the pre-training dataset (4.4M and 43.4M tiles), and its diversity (colon-specific and pan-cancer). The model trained on 43.4 million tiles using ViT-B/16 is referred to as \textbf{Phikon}.

% RudolfV和Hibou都是从数据集的角度出发，用了更大且更diversity的数据集。其中RudolfV在构建数据集时引入了病理学家的专业知识；Hibou在构建数据集时采用了类似lunit的Data Augmentations方法（Random angle rotation，Random horizontal and vertical flips，RandStainNA ，Color jittering）使得数据集更加丰富
%Virchow2：更大，更多样的数据集 + Pathology-adapted training method：①Domain-specific augmentations（Mixed magnification，Extended-Context Translation，Photometric Augmentations）② 用the kernel density estimator (KDE)作为entropy estimator代替DINOv2原来用的KoLeo. 还有俩变体：使用ViT-G/14的Virchow2G和其使用ViT-S/14的Distillation版本Virchow2G Mini
% Phikon-v2 除了数据集来源更多看不出来有啥好的。。

\textcolor{red}{[To be improved]} \textbf{Virchow} \cite{Virchow}, \textcolor{red}{RudolfV} \cite{RudolfV} , \textcolor{red}{Hibou} \cite{Hibou}, \textcolor{red}{Virchow2} \cite{Virchow2}, \textcolor{red}{Phikon-v2} \cite{Phikon-v2} and \textbf{UNI} \cite{UNI} all utilizes SSL framework powered by DINOv2 \cite{DINOv2} to train a ViT model. DINOv2 follows a student-teacher paradigm, where the student encoder is trained on noisy input tiles (including masked global crops and local crops) to align with the teacher encoder, which processes global crops and is updated through exponential moving average (EMA). The difference is Virchow trains the ViT-H model on 1.5 million H\&E WSIs collected from the Memorial Sloan Kettering Cancer Center (MSKCC), while UNI trains the ViT-L model on a curated pre-training dataset consisting of over 100 million tissue patches from 100,000 diagnostic H\&E WSIs sourced from the GTEx collection, along with data from two proprietary hospitals: Massachusetts General Hospital (MGH) and Brigham and Women’s Hospital (BWH).

\textbf{\textit{Campanella et al.}}~\cite{campanella2024computational} compare the performance of masked autoencoders (MAE) \cite{MAE} and DINO on millions of tiles derived from over 423,000 pathology slides. They employe three pretraining settings: using ViT-S and ViT-B model pretrained on 1.6 million tiles under DINO framework, and using ViT-L model pretrained on 3.2 million tiles with MAE framework. Their results demonstrate the superiority of DINO when applied to pretraining foundation models in pathology.

\textit{\textbf{Aben et al.}}~\cite{Kaiko} develope the \textit{Online Patching} method during the pretraining process, which allows for the online high-throughput extraction of patches of arbitrary size and resolution from WSIs stored in blob storage. This method addresses the issue of requiring dataset recreation for new requirements (such as the size and FoV of tile) after the dataset has been created, and also saving storage resources. The proposed method, \textbf{Kaiko}, trains multiple ViT models of different scales using Online Patching within the frameworks of DINO and DINOv2.

\textbf{GigaPath} \cite{GigaPath} is a whole-slide pathology foundation model trained on 171,189 WSIs from Providence Health System (PHS). It trains a ViT-G/14 as the tile-level encoder under the DINOv2 framework, and then trains a LongNet \cite{LongNet} as the slide-level encoder to get the embedding of whole slide. The model first divides the whole slide into a sequence of image tiles, and then uses the tile-level encoder to learn the representation of each tile, treating them as visual tokens. This turns a slide into a long sequence of tokens, which is then fed into LongNet to obtain the overall slide representation. LongNet utilizes its \textit{Dilated Attention} mechanism to perform sparse attention computation, which reduces the computational complexity to linear.


\subsection{Multi-Modal}

Summary


\textbf{PLIP} \cite{PLIP} fine-tunes the pretrained contrastive language–image pretraining (CLIP) model \cite{CLIP} on a dataset consisting of 208,414 pathology tile-caption pairs. Through contrastive loss, it ensures that the embeddings encoded by the text encoder and image encoder are as similar as possible for the paired tile and caption, and as dissimilar as possible for the non-paired tile and caption. This approach enhances the model's understanding of pathology tiles, thereby facilitating multiple downstream applications.

\textbf{CONCH} \cite{CONCH} is pre-trained on over 1.17 million image-caption pairs using the CoCa framework \cite{CoCa}. This architecture extends CLIP by adding a multimodal decoder that takes image embeddings as input and outputs text embeddings. In addition to the contrastive loss for aligning the image and text modalities, a captioning loss is incorporated to predict image captions.

\textbf{PRISM} \cite{PRISM} is a multi-modal slide-level foundation model that consists of a slide encoder and a language decoder. It first performs tile-level embedding of WSIs using Virchow and further obtains slide-level representations through the slide encoder which is implemented by the Perceiver network \cite{Perceiver}. Then, clinical reports rewritten by GPT-4 \cite{GPT-4} are encoded using pre-trained BioGPT \cite{BioGPT}. The model is trained on slide-level data from both modalities within the CoCa framework. Its main objectives are twofold: (1) to align the encoded report embedding with the slide embedding, and (2) to match the caption generated by BioGPT with the rewritten ground-truth report.

\textbf{CHIEF} \cite{CHIEF} learns slide-level representations and utilizes anatomical site information as textual input to obtain rich multi-modal representations. The pre-training process is divided into two stages: (1) pre-training a text encoder (directly using CLIP's text encoder) and an image encoder (trained using CTransPath on 15 million tiles), and then (2) using the text encoder to encode the anatomical site to obtain text features, while the image encoder encodes the tiles sequence extracted from WSIs to obtain WSI-level features. These two types of features are subsequently combined through attention-based feature fusion, supported by instance-level feature identification and contrastive learning at the WSI level.

\textbf{PathChat} \cite{PathChat}, unlike other foundational models that focus on extracting features from pathology images, is a pathology-focused MLLM. To encode both images and text simultaneously, it uses UNI as the image encoder and further adopts a method similar to CONCH for vision-language pretraining. The trained vision encoder is then connected to Llama 2 \cite{Llama2} and fine-tuned using 456,916 instructions, which include various types such as conversations, descriptions, and multiple-choice questions.

\textbf{TITAN} \cite{TITAN} is a multi-modal whole-slide foundation model primarily aimed at training a slide encoder. Its pretraining is divided into three stages. In the first stage, TITAN uses a patch encoder to encode each patch of a WSI. The training is conducted within the iBOT framework, incorporating semantic encoding to account for the spatial significance of different patches. The second and third stages use the encoder trained in the first stage and are carried out under the CoCa framework. These stages leverage over 423,000 tile-caption pairs generated by PathChat and more than 182,862 WSI-report pairs to enhance the model's language capabilities. This progression, from local to global training, helps gradually build the model's ability to comprehend and generate meaningful vision-language representations for WSIs.


% 临时存一下：

\begin{table*}[ht]
\centering
\scriptsize
\setlength\tabcolsep{2pt}
\caption{Statistics of Datasets Used for Pre-training CPath Foundation Models}
\begin{threeparttable}
\begin{tabular}{ccccccccccccccccc}
\toprule
& \multirow{2}{*}{\textbf{Dataset}} &\multicolumn{2}{c}{\textbf{Data Sources}} & \multirow{2}{*}{\textbf{\# WSIs}} & \multirow{2}{*}{\textbf{\# Tiles}} & \multirow{2}{*}{\textbf{Image Size}} & \textbf{Field of View} & \multicolumn{3}{c}{\textbf{Staining Types}} & \multicolumn{2}{c}{\textbf{Data Used By}} \\ 
\specialrule{0em}{0pt}{-0.2pt}
\cmidrule(lr){3-4} \cmidrule(lr){9-11} \cmidrule(lr){12-13}

\specialrule{0em}{-1pt}{0pt}
&& \textbf{Public} & \textbf{Private}  & & & & \textbf{(FoV)} & \textbf{H\&E} & \textbf{IHC} & \textbf{Others} & \textbf{Method} & \textbf{Reference} \\ 

\specialrule{0em}{-0.2pt}{0pt}
\midrule

\multirow{20}{*}{\makecell[c]{\rotatebox{90}{\textbf{Uni-modal}}}} & - &TCGA, PAIP & -  & 32.2K & 15.6M & 1024$\times$1024 & 20$\times$ & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & CTransPath &\cite{CTransPath} \\ 
\cmidrule(r){2-13}
&& TCGA & JFT54 & 29.0K & 50.0M & 224$\times$224 & 20$\times$ & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & REMEDIS & \cite{REMEDIS} \\ \cmidrule(r){2-13}
&&TCGA & TULIP & 36.7K & 32.6M & 512$\times$512 & \{20, 40\}$\times$ & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & Lunit DINO & \cite{Lunit} \\ \cmidrule(r){2-13}
&&TCGA & - &6.1K & 43.4M & 224$\times$224 & 20$\times$ & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & Phikon & \cite{Phikon} \\ \cmidrule(r){2-13}

&&- & MSKCC  & 1.5M & 2.0B & 224$\times$224 & 20$\times$ & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} &Virchow & \cite{Virchow}   \\ \cmidrule(r){2-13}

% UNI & U & 100K & 100M & 256$\times$256, 512$\times$512 & 20$\times$ & H\&E &  MGH*, BWH*, GTEx  \\ 

&&- & MSHS   & 423K & 1.6B, 3.2B & 224$\times$224 & 20$\times$ & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & - & \cite{campanella2024computational}\\ \cmidrule(r){2-13}
&&TCGA & Proprietary & 134K & 1.2B &  256$\times$256 & \{20, 40, 80\}$\times$ & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & RudolfV & \cite{RudolfV}   \\ \cmidrule(r){2-13}
&& TCGA & - & 29.0K & 256M & 256$\times$256 & \{5, 10, 20, 40\}$\times$ & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & Kaiko & \cite{Kaiko}  \\ \cmidrule(r){2-13}
&&- &  PHS& 171K & 1.4B &  256$\times$256 & 20$\times$ & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & GigaPath & \cite{GigaPath}\\ \cmidrule(r){2-13}
&&- & Proprietary& 1.1M & 512M, 1.2B &  224$\times$224 & 20$\times$ & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} &  Hibou & \cite{Hibou}\\ \cmidrule(r){2-13}
&&  - & MSKCC & 3.1M & 2.0B &  392$\times$392 & \{5, 10, 20, 40\}$\times$ & \textcolor{green}{\ding{51}}  & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} &Virchow2 & \cite{Virchow2}\\ \cmidrule(r){2-13}
&&TCGA, GTEx, \textit{etc.} & Proprietary$\times$4 & 58.0K & 456M & 224$\times$224 & 20$\times$ & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & Phikon-v2 & \cite{Phikon-v2} \\ \cmidrule(r){2-13}
&& GTEx & MGH, BWH  & 100K & 100M & 256$\times$256, 512$\times$512 & 20$\times$ & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & UNI & \cite{UNI}\\ 

\midrule
\midrule

\multirow{16}{*}{\makecell[c]{\rotatebox{90}{\textbf{Multi-modal}}}} & & Twitter, PathLAION & - & - & 208K & 224$\times$224 & - & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & - & PLIP & \cite{PLIP} \\
\cmidrule(r){2-13}
&&PMC OA & LBC & - & 207K & - & - &\textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & PathCLIP & \cite{PathCLIP}\\ 
\cmidrule(r){2-13}
&&PMC OA & LBC & - & - & - & - &\textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & PathAsst & \cite{PathCLIP}\\ 
\cmidrule(r){2-13}
&& - &Proprietary   & 21K & 16M & 256$\times$256  & 20$\times$ & \textcolor{green}{\ding{51}} &  - &- &\multirow{2}{*}{CONCH} & \multirow{2}{*}{\cite{CONCH}}\\
&&PMC OA & EDU& - & 1.17M & 448$\times$448 & - & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & & \\ 
\cmidrule(r){2-13}
&&TCGA & Proprietary & 587K & $>$500K & 224$\times$224 & 20$\times$  & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & PRISM & \cite{PRISM} \\ 
% CHIEF &  tiles; 60K WSIs-anatomical sites pairs & H\&E & TCGA, \textit{Proprietary}*, etc.\\ 
\cmidrule(r){2-13}
% &\multirow{2}{*}{CHIEF} & \multirow{2}{*}{\cite{CHIEF}} & 32.2K & 15.6M & 256$\times$256 & 10$\times$ & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & TCGA, PAIP & - \\ 
&&TCGA, GTEx, \textit{etc.} & Proprietary & 60K & - & 256$\times$256 & 10$\times$ & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & CHIEF  & \cite{CHIEF} \\ 
\cmidrule(r){2-13}
% &\multirow{2}{*}{PathChat} & \multirow{2}{*}{\cite{PathChat}} & 100K & 100M & 256$\times$256 & 20$\times$ & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} &  GTEx & MGH, BWH \\ 
&&PMC OA & EDU & - & 1.18M & 448$\times$448 & - & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} &\multirow{2}{*}{PathChat} & \multirow{2}{*}{\cite{PathChat}} \\
&&PMC OA, TCGA & Proprietary& - & -  & - & - & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} &  & \\ 
\cmidrule(r){2-13}
&&GTEx &  Proprietary& 336K & - & 512$\times$512 & 20$\times$ & \textcolor{green}{\ding{51}}  &  \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & \multirow{3}{*}{TITAN} & \multirow{3}{*}{\cite{TITAN}} \\ 
&&GTEx &  Proprietary & - & 423K & 8192$\times$8192 & 20$\times$ & \textcolor{green}{\ding{51}}  &  \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} &  & \\ 
&&GTEx &  Proprietary&183K & - &32768$\times$32768 & - &\textcolor{green}{\ding{51}} &\textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & & \\ 

\bottomrule
\end{tabular}
% \begin{tablenotes}

%     \end{tablenotes}
\end{threeparttable}

\label{tab:datasets}

\end{table*}

==> sections/methods_v2.tex <==

% \begin{table*}[ht]
% \centering
% \scriptsize
% \setlength\tabcolsep{2pt}
% \begin{threeparttable}

% \caption{Comparative Overview of CPath Foundation Models}
% \label{tab:methods}
% \begin{tabular}{cccccccccc}
% \toprule
% % \textbf{} & \textbf{Method} & \textbf{SSL Framework} & \textbf{Visual (\& Language) Backbone [\# Param.]}  & \textbf{Image Type}\tnote{$\dagger$} \\
% % text backbone to be supplied！！！！！！！！！！！！！！！！！！
% \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Reference}} &\textbf{SSL}  & \multicolumn{2}{c}{\textbf{Backbone\tnote{$\dagger$}\;\;[\# Param. (\textcolor{orange}{Training / Tuning}, \textcolor{blue!80}{Frozen})]}} & \textbf{Input } & \multicolumn{2}{c}{\textbf{Pre-training Strategy\tnote{$\ddagger$}}} \\ 

% \specialrule{0em}{0pt}{-0.2pt}
% \cmidrule(lr){5-6} \cmidrule(lr){8-9}
% \specialrule{0em}{-1pt}{0pt}

%  &  &  & \textbf{Framework} & \textbf{Vision} & \textbf{Language}  & \textbf{Type} &  \textbf{Vision} & \textbf{Language}\\ 

% \midrule
% \multirow{20}{*}{\makecell[c]{\rotatebox{90}{\textbf{Uni-modal}}}} & CTransPath & \cite{CTransPath} & MoCo v3 & Swin Transformer [28M \textcolor{orange}{\ding{108}}] & - & Tile & S & -\\ \cmidrule(r){2-9}
%     & REMEDIS & \cite{REMEDIS} & SimCLR  &  ResNet-152 (2$\times$) [232M \textcolor{orange}{\ding{108}}] & - & Tile & D & -\\ \cmidrule(r){2-9}
%     & Lunit DINO & \cite{Lunit} & DINO  & ViT-S/(8,16) [22M \textcolor{orange}{\ding{108}}] & - & Tile & S & -\\ \cmidrule(r){2-9}
%     & Phikon & \cite{Phikon} & iBOT & ViT-B/16 [86M \textcolor{orange}{\ding{108}}] & - & Tile & S & -\\ \cmidrule(r){2-9}
    
%     & Virchow & \cite{Virchow} & DINOv2 & ViT-H/14 [632M \textcolor{orange}{\ding{108}}] & - & Tile  & S & -\\ \cmidrule(r){2-9}
%     & \multirow{2}{*}{-} & \multirow{2}{*}{\cite{campanella2024computational}} & DINO & ViT-S [22M \textcolor{orange}{\ding{108}}], ViT-B [86M \textcolor{orange}{\ding{108}}] & - & \multirow{2}{*}{Tile}  & \multirow{2}{*}{S} & -\\
%     & & & MAE & ViT-L [307M \textcolor{orange}{\ding{108}}] & - & && -\\ \cmidrule(r){2-9}
%     & RudolfV & \cite{RudolfV} & DINOv2 & ViT-L/14 [307M \textcolor{orange}{\ding{108}}] & - & Tile  & D & -\\ \cmidrule(r){2-9}
%     & \multirow{2}{*}{Kaiko} & \multirow{2}{*}{\cite{Kaiko}} & DINO & ViT-S/(8,16) [22M \textcolor{orange}{\ding{108}}], ViT-B/(8,16) [86M \textcolor{orange}{\ding{108}}] & - & \multirow{2}{*}{Tile}  & \multirow{2}{*}{D}& -\\
%     &  & & DINOv2 & ViT-L/14 [307M \textcolor{orange}{\ding{108}}] & -&   &\\ \cmidrule(r){2-9}
%     & GigaPath & \cite{GigaPath} & DINOv2 & ViT-G/14 [1.1B \textcolor{orange}{\ding{108}}] \& LongNet [125M \textcolor{orange}{\ding{108}}] & -& WSI & S & -\\ \cmidrule(r){2-9}
%     & Hibou & \cite{Hibou} & DINOv2 & ViT-B/14 [86M \textcolor{orange}{\ding{108}}], ViT-L/14 [307M \textcolor{orange}{\ding{108}}] & -& Tile & S & -\\ \cmidrule(r){2-9}
%     & Virchow2 & \cite{Virchow2} & DINOv2 & ViT-B/16 [86M \textcolor{orange}{\ding{108}}] & - & Tile & S & -\\  \cmidrule(r){2-9}
%     & Phikon-v2 & \cite{Phikon-v2} & DINOv2 & ViT-L/16 [307M \textcolor{orange}{\ding{108}}] & - & Tile & S& -\\ \cmidrule(r){2-9}

%     & UNI & \cite{UNI} & DINOv2 & ViT-L/16 [307M \textcolor{orange}{\ding{108}}] & - & Tile  & S & -\\ 
%     \midrule
%     \midrule
    
% % \multirow{4}{*}{\makecell[c]{\rotatebox{90}{\textbf{Multi-modal}}}} & PLIP \cite{PLIP} & CLIP & ViT-B/32 [86M] \& \textcolor{red}{CLIP Text Encoder [76M]} & T  &\\
% %     & CONCH \cite{CONCH} & CoCa & ViT-B/16 [86M] \& 12 Transformer Layers (2$\times$)  [14M] & T &\\
% %     & PRISM \cite{PRISM} & CoCa & ViT-H/14 [632M] + Perceiver [105M] \& BioGPT [345M] & S &\\ 
    
% %     & PathChat \cite{PathChat} & DINOv2, CoCa & 1 & T &\\ 
% %     & CHIEF \cite{CHIEF} & CLIP & Swin Transformer [28M] \& CLIP Text Encoder [76M]  & S &\\ 

% \multirow{10}{*}{\makecell[c]{\rotatebox{90}{\textbf{Multi-modal}}}} & PLIP & \cite{PLIP} & CLIP & ViT-B/32 [86M \textcolor{orange}{\ding{108}}] & \textcolor{red}{CLIP Text Encoder [76M \textcolor{orange}{\ding{108}}]} & Tile & D & N \\ \cmidrule(r){2-9}
%     & PathCLIP & \cite{PathCLIP}& CLIP &  ViT-B/32 [86M \textcolor{orange}{\ding{108}}] & \textcolor{red}{CLIP Text Encoder [76M \textcolor{orange}{\ding{108}}]} & Tile & D & N \\ \cmidrule(r){2-9}
    
%     & PathAsst & \cite{PathCLIP} & CLIP & ViT-B/32 [86M \textcolor{iceblue!300}{\ding{108}}] & Vicuna-13B [13B \textcolor{orange}{\ding{108}}] & Tile & F & I \\ \cmidrule(r){2-9}
    
%     & CONCH & \cite{CONCH} & CoCa, iBOT & ViT-B/16 [86M \textcolor{orange}{\ding{108}}] & Transformer Layers [$\sim$14M \textcolor{orange}{\ding{108}}] & Tile & S & N \\ \cmidrule(r){2-9}
%     % 如果一个方法的vision部分来自off the shelf，那么就不认为这个算他的一个stage，相应的方法和数据集都视为没有
%     & PRISM & \cite{PRISM} & CoCa & ViT-H/14 [632M \textcolor{iceblue!300}{\ding{108}}] \& Perceiver Net. [105M \textcolor{orange}{\ding{108}}] & BioGPT [345M \textcolor{orange}{\ding{108}}, 172M \textcolor{iceblue!300}{\ding{108}}] & WSI & F, S & N, F\\ \cmidrule(r){2-9} 
    
%     & CHIEF & \cite{CHIEF} & CLIP, MoCo v3 & Swin Transformer [28M] &  & WSI & & -\\ \cmidrule(r){2-9}
%     & PathChat & \cite{PathChat} & CoCa, DINOv2 & ViT-L/16 [307M] &  & Tile & & -\\ \cmidrule(r){2-9} 
    
%     & TITAN & \cite{TITAN} & CoCa, iBOT &  ViT-S [22M] & CLIP Text Encoder [76M] & WSI && -\\ \bottomrule
% \end{tabular}
% \begin{tablenotes}
%     % \item[$\dagger$] The abbreviations stand for uni-modal (U) and multi-modal (M).
%     \item[$\dagger$] For simplicity, we have streamlined some expressions. For example, ``/8" denotes a patch size of 8$\times$8 pixels, and ``/(8,16)" represents ``/8" and ``/16", respectively.
%     \item[$\ddagger$] There are five training strategies: frozen (F), from scratch (S), domain-specific tuning (D), instruction tuning (I), and non-instruction tuning (N).
%     \end{tablenotes}
% \end{threeparttable}
% \end{table*}

\begin{table*}[ht]
\centering
\scriptsize
\setlength\tabcolsep{3.5pt}
\begin{threeparttable}

\caption{Overview of training strategies of CPathFMs}
\vspace{-5mm}
\label{tab:methods}
\begin{tabular}{cccccccccc}
\toprule
\multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Reference}} &\textbf{SSL}  & \multicolumn{2}{c}{\textbf{Backbone [\# Param.]\tnote{$\dagger$}}} & \textbf{Input } & \multicolumn{2}{c}{\textbf{Pre-training Strategy\tnote{$\ddagger$}}} \\ 

\specialrule{0em}{0pt}{-0.2pt}
\cmidrule(lr){5-6} \cmidrule(lr){8-9}
\specialrule{0em}{-1pt}{0pt}

 &  &  & \textbf{Framework} & \textbf{Vision} & \textbf{Language}  & \textbf{Images} &  \textbf{Vision} & \textbf{Language}\\ 

\midrule
\multirow{20}{*}{\makecell[c]{\rotatebox{90}{\textbf{Uni-modal}}}} & CTransPath & \cite{CTransPath} & MoCo v3 & Swin Transformer [\textcolor{orange}{28M}] & - & Tiles & S & -\\ \cmidrule(r){2-9}
    & REMEDIS & \cite{REMEDIS} & SimCLR  &  ResNet-152 (2$\times$) [\textcolor{orange}{232M}] & - & Tiles & D & -\\ \cmidrule(r){2-9}
    & Lunit DINO & \cite{Lunit} & DINO  & ViT-S/(8,16) [\textcolor{orange}{22M}] & - & Tiles & S & -\\ \cmidrule(r){2-9}
    & Phikon & \cite{Phikon} & iBOT & ViT-B/16 [\textcolor{orange}{86M}] & - & Tiles & S & -\\ \cmidrule(r){2-9}
    
    & Virchow & \cite{Virchow} & DINOv2 & ViT-H/14 [\textcolor{orange}{632M}] & - & Tiles  & S & -\\ \cmidrule(r){2-9}
    & \multirow{2}{*}{-} & \multirow{2}{*}{\cite{campanella2024computational}} & DINO & ViT-S [\textcolor{orange}{22M}], ViT-B [\textcolor{orange}{86M}] & - & \multirow{2}{*}{Tiles}  & \multirow{2}{*}{S} & -\\
    & & & MAE & ViT-L [\textcolor{orange}{307M}] & - & && -\\ \cmidrule(r){2-9}
    & RudolfV & \cite{RudolfV} & DINOv2 & ViT-L/14 [\textcolor{orange}{307M}] & - & Tiles  & D & -\\ \cmidrule(r){2-9}
    & \multirow{2}{*}{Kaiko} & \multirow{2}{*}{\cite{Kaiko}} & DINO & ViT-S/(8,16) [\textcolor{orange}{22M}], ViT-B/(8,16) [\textcolor{orange}{86M}] & - & \multirow{2}{*}{Tiles}  & \multirow{2}{*}{D}& -\\
    &  & & DINOv2 & ViT-L/14 [\textcolor{orange}{307M}] & -&   &\\ \cmidrule(r){2-9}
    & GigaPath & \cite{GigaPath} & DINOv2 & ViT-G/14 [\textcolor{orange}{1.1B}] \& LongNet [\textcolor{orange}{125M}] & -& WSIs & S, S & -\\ \cmidrule(r){2-9}
    & Hibou & \cite{Hibou} & DINOv2 & ViT-B/14 [\textcolor{orange}{86M}], ViT-L/14 [\textcolor{orange}{307M}] & -& Tiles & S & -\\ \cmidrule(r){2-9}
    & Virchow2 & \cite{Virchow2} & DINOv2 & ViT-B/16 [\textcolor{orange}{86M}] & - & Tiles & S & -\\  \cmidrule(r){2-9}
    & Phikon-v2 & \cite{Phikon-v2} & DINOv2 & ViT-L/16 [\textcolor{orange}{307M}] & - & Tiles & S& -\\ \cmidrule(r){2-9}

    & UNI & \cite{UNI} & DINOv2 & ViT-L/16 [\textcolor{orange}{307M}] & - & Tiles  & S & -\\ 
    \midrule
    \midrule
\multirow{10}{*}{\makecell[c]{\rotatebox{90}{\textbf{Multi-modal}}}} & PLIP & \cite{PLIP} & CLIP & ViT-B/32 [\textcolor{orange}{86M}] & Transformer Layers [\textcolor{orange}{63M}] & Tiles & D & N \\ \cmidrule(r){2-9}
    & PathCLIP & \multirow{2}{*}{\cite{PathCLIP}}& \multirow{2}{*}{CLIP} &  ViT-B/32 [\textcolor{orange}{86M}] & Transformer Layers [\textcolor{orange}{63M}] & Tiles & D & N \\ 
    
    \specialrule{0em}{0pt}{0.2pt}
% \cmidrule(lr){5-9} 
% \specialrule{0em}{-1pt}{0pt}
    
    & PathAsst & & & ViT-B/32 [\textcolor{blue!80}{86M}] & Vicuna-13B [\textcolor{orange}{13B}] & Tiles & F & I \\ \cmidrule(r){2-9}
    
    & CONCH & \cite{CONCH} & CoCa, iBOT & ViT-B/16 [\textcolor{orange}{86M}] & Transformer Layers [\textcolor{orange}{$\sim$86M}] & Tiles & S & N \\
    \cmidrule(r){2-9}
    % 如果一个方法的vision部分来自off the shelf，那么就不认为这个算他的一个stage，相应的方法和数据集都视为没有
    & PRISM & \cite{PRISM} & CoCa & ViT-H/14 [\textcolor{blue!80}{632M}] \& Perceiver Net. [\textcolor{orange}{105M}] & BioGPT [\textcolor{orange}{345M}, \textcolor{blue!80}{172M}] & WSIs & F, S & N, F\\ \cmidrule(r){2-9} 
    
    & CHIEF & \cite{CHIEF} & CLIP & Swin Transformer [\textcolor{orange}{28M}] & Transformer Layers [\textcolor{orange}{63M}] & WSIs & D & N \\ \cmidrule(r){2-9}
    & PathChat & \cite{PathChat} & CoCa & ViT-L/16 [\textcolor{orange}{307M}] &  Llama 2 [\textcolor{orange}{13B}] & Tiles & D & I \\ \cmidrule(r){2-9} 
    
    & TITAN & \cite{TITAN} & CoCa, iBOT &  ViT-B/16 [\textcolor{blue!80}{86M}] \& ViT-S [\textcolor{orange}{22M}] & Transformer Layers [\textcolor{orange}{$\sim$86M}]  & WSIs & F, S & N\\
\bottomrule
\end{tabular}

\begin{tablenotes}
        \item[$\dagger$] For simplicity, we have streamlined some expressions. For example, ``/8" denotes a patch size of 8$\times$8 pixels, and ``/(8,16)" represents ``/8" and ``/16", respectively. \\ The \textbf{\textcolor{orange}{orange}} color in [ ] represents the parameters that are being trained or tuned, while the \textbf{\textcolor{blue!80}{blue}} color represents the frozen parameters.

        \item[$\ddagger$] Pre-training strategies: \textbf{F}: Frozen, \textbf{S}: From Scratch, \textbf{D}: Domain-Specific Tuning, \textbf{I}: Instruction Tuning, \textbf{N}: Non-instruction Tuning.
    % \item[$\ddagger$] There are five training strategies: frozen (F), from scratch (S), domain-specific tuning (D), instruction tuning (I), and non-instruction tuning (N).
\end{tablenotes}
\end{threeparttable}
\vspace{-3mm}
\end{table*}




% \begin{table*}[ht]
% \centering
% \begin{threeparttable}
% \begin{tabular}{cccccccc}
% \toprule
% \textbf{Method} & \textbf{\# Slide-Report}\tnote{$\dagger$} & \textbf{\# Tile-Caption} & \textbf{Tile Size} & \textbf{FoV} & \textbf{Staining Type} & \textbf{Source} \\ \midrule


% PLIP & \textbf{-} & 208K & $\text{224}^{\text{2}}$ & Various & \textcolor{red}{H\&E} & Twitter, PathLAION \\ 
% PRISM & 587K-195K & \textbf{-} & $\text{224}^{\text{2}}$ & 20$\times$ & H\&E & TCGA, \textit{Proprietary}* \\ 

% PathChat & \textbf{-} &  & $\times$ &  &  & \\ 

% CHIEF &  &  & $\text{256}^{\text{2}}$ & 10$\times$ &  & \\ 


% % remember the source dataset citation


% \bottomrule
% \end{tabular}
% \begin{tablenotes}
%     \item[$\dagger$] Note that one or more WSIss usually have a corresponding clinical report in practice.
%     \item[$\ast$] Internally collected dataset.
%     \end{tablenotes}
% \end{threeparttable}

% \caption{Pre-training datasets for multi-modal methods}
% \label{tab:pre-train-datasets-multi}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \begin{threeparttable}
% \begin{tabular}{ccccc}
% \toprule
% \textbf{Method} & \textbf{Statistical Description}\tnote{$\dagger$}  & \textbf{Staining Type} & \textbf{Source} \\ \midrule


% PLIP &  208K tile-caption pairs & \textcolor{red}{H\&E} & Twitter, PathLAION \\ 
% PathCLIP &  207K tile-caption pairs & H\&E, IHC & PubMed, LBC* \\ 
% PathAsst &  180K; 35K instruction-following pairs & H\&E, IHC & PubMed, LBC*  \\ 
% CONCH & 1.17M tile-caption pairs & H\&E, IHC, special & PMC OA, EDU*\\ 
% PRISM & 587K WSIss + 195K clinical reports\tnote{$\ddagger$} & H\&E & TCGA, \textit{Proprietary}* \\ 

% CHIEF & 15.6M tiles; 60K WSIs-anatomical sites pairs & H\&E & TCGA, \textit{Proprietary}*, etc.\\ 

% PathChat & \makecell[c]{100M tiles; 1.2M tile-caption pairs; 467K instructions}    & H\&E, IHC & \makecell[c]{PubMed, TCGA, \textit{Proprietary}*}\\ 

% TITAN & 336K WSIs; 423K tile-caption pairs; 183K WSI-report pairs & H\&E, IHC & TCGA, \textit{Proprietary}*, etc.\\ 


% % remember the source dataset citation


% \bottomrule
% \end{tabular}
% \begin{tablenotes}
%     \item[$\dagger$] Multimodal foundation models are typically trained in several stages, with different stages of data separated by semicolons (";").
%     \item[$\ddagger$] Note that one or more WSIs usually have a corresponding clinical report in practice.
%     \item[$\ast$] Internally collected dataset.
%     \end{tablenotes}
% \end{threeparttable}

% \caption{Pre-training datasets for multi-modal methods.}
% \label{tab:pre-train-datasets-multi}
% \end{table*}

% \textcolor{blue}{Self-supervised learning (SSL)} 
SSL
has been widely applied in the development of CPathFMs to address the lack of labels. These methods typically adapt SSL frameworks that have proven successful in natural images and perform pre-training on carefully curated pathology datasets. Depending on the type of pathology data they used, these approaches can be categorized into uni-modal and multi-modal methods, which are summarized in Table~\ref{tab:methods}.

% \subsection{Data Curation}


\subsection{Uni-Modal CPathFMs}

Uni-modal CPathFMs are generally trained on large,  domain-specific pathology datasets using self-supervised contrastive learning frameworks to learn robust representations of pathological images without labeled data. These methods often apply two different data augmentations to an image tile and maximize the mutual information between the augmented views to train a visual feature extractor. 
Similar to the development of contrastive learning in natural images, CPathFMs were initially proposed within the MoCo \cite{MoCo3} and SimCLR \cite{SimCLR} frameworks. 
% Following a transition through the DINO \cite{DINO}, DINOv2 \cite{DINOv2} 
% was ultimately established 
% as the primary framework, around which numerous subsequent studies have been developed.
Following a transition through the DINO \cite{DINO}, DINOv2 \cite{DINOv2} 
was established  
as the leading framework, 
serving as the foundation for numerous subsequent studies.

\textbf{DINO-based CPathFMs.}
To address the instability during 
% \textcolor{blue}{Vision Transformer (ViT)} 
ViT
training, DINO, which follows a student-teacher paradigm, performs self-distillation in a self-supervised manner. Specifically, it matches the output of the student network with the output of the teacher network after centering (an operation similar to batch normalization) and updates the teacher network using exponential moving average (EMA) \cite{MoCo}. 
As a successful application of SSL on ViT, DINO has been adopted as a framework for training CPathFMs. 
% Campanella~\textit{et al.}~\shortcite{campanella2024computational} compared the performance of masked autoencoders (MAE) \cite{MAE} and DINO on different scales of pathology datasets and ViT models, 
% 
Campanella~\textit{et al.}~\shortcite{campanella2024computational} compared the performance of DINO and masked autoencoders (MAE) \cite{MAE} on different scales of pathology datasets, 
ultimately demonstrating the superiority of DINO for pre-training CPathFMs. 
Kang~\textit{et al.}~\shortcite{Lunit} focused on domain-aligned pre-training and proposed data augmentation and curation strategies specifically for pathological images.

\textbf{DINOv2-based CPathFMs.}
Filiot \textit{et al.}~\shortcite{Phikon} trained a ViT within the iBOT framework \cite{iBOT} using Masked Image Modeling (MIM). This approach involves randomly masking certain regions and reconstructing the masked areas to learn valuable representations for a given image tile.

As an improved version of DONO, DINOv2 incorporates MIM and replaces the centering with Sinkhorn-Knopp \cite{SwAV} for normalization. 
Most studies using the DINOv2 framework, such as UNI \cite{UNI}, mainly focus on larger ViT models and more extensive and diverse pre-training datasets. Among them, RudolfV \cite{RudolfV} incorporates the domain knowledge of pathologists in dataset construction. 
Some methods have adopted pathology-adapted training methods within the DINOv2 framework, such as Aben \textit{et al.}~\shortcite{Kaiko} who developed the Online Patching method during the pre-training process, allowing for the online high-throughput extraction of patches of arbitrary size and resolution. Additionally, Virchow2 \cite{Virchow2} replaces the original entropy estimator in DINOv2 with the kernel density estimator (KDE).
Unlike previous methods, GigaPath focuses on learning the representation of whole-slide images. It first uses the tile-level encoder, trained under the DINOv2 framework, to learn the representation of a sequence of image tiles obtained by dividing the whole slide, treating them as visual tokens. These tokens are then fed into LongNet \cite{LongNet}, which utilizes its Dilated Attention mechanism to perform sparse attention computation, thereby obtaining the overall slide representation.


\textbf{Other Uni-Modal CPathFMs.}
While the majority of uni-modal methods focus on DINO and DINOv2, some methods employ other SSL frameworks. CTransPath \cite{CTransPath} adds a branch to MoCov3 to generate queries that retrieve semantically similar samples from the memory bank as positive samples, thus guiding the network's training with a semantically relevant contrastive loss.
REMEDIS \cite{REMEDIS} transfers a ResNet model, pre-trained on large-scale natural images, to the SimCLR framework for self-supervised training on pathological images.

\subsection{Multi-Modal CPathFMs}

Multi-modal CPathFMs enhance the model’s understanding of pathological images by aligning paired image-text data under the visual-language multi-modal SSL frameworks, such as CLIP \cite{CLIP} and CoCa \cite{CoCa}. 
These methods typically train pre-trained uni-modal modules using uni-modal SSL frameworks before performing joint visual-language pre-training, which has been shown to improve the performance of downstream tasks \cite{lu2023visual}.
Moreover, multi-modality provides an extra perspective for CPathFMs, where pathological visual representations aligned with additional language signals in latent space can assist large language models (LLMs) in understanding pathology knowledge, thereby contributing to the construction of generative foundation AI assistants for pathologists~\cite{PathChat}.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{imgs/EvaTasks.pdf}
    \vspace{-8mm}
    \caption{Taxonomy of evaluation tasks for pre-trained CPathFMs. Uni-modal and multi-modal CPathFMs are highlighted in \textcolor[rgb]{0.439, 0.188, 0.627}{\textbf{purple}} and \textcolor[rgb]{0.851,0,0}{\textbf{red}}, respectively.}
    \vspace{-3mm}
    \label{fig:evaluation-tasks}
\end{figure*}

\textbf{CLIP-based CPathFMs.}
CLIP ensures that the embeddings generated by the image encoder and text encoder are as similar as possible for paired image-text data by utilizing contrastive loss.
PLIP \cite{PLIP} and PathCLIP \cite{PathCLIP} both fine-tune a pre-trained CLIP model using datasets composed of paired tiles and their captions. 
PathAsst \cite{PathCLIP} leverages PathCLIP as the visual component to build a pathological multi-modal large language model (MLLM). It first trains a fully connected layer between the visual component and the LLM using instructions constructed from question-answer pairs to align the image encoder with the LLM. Then, the LLM is fine-tuned with a small number of instructions.
CHIEF \cite{CHIEF} uses an image encoder from CTransPath to encode the tile sequence extracted from WSIs to obtain WSI-level features and encodes anatomical site information as textual features using the original CLIP's text encoder. The two are combined to obtain rich WSI-level multi-modal representations.


\textbf{CoCa-based CPathFMs.}
CoCa \cite{CoCa} extends CLIP by adding a multi-modal decoder that takes image embeddings as input and outputs text embeddings. In addition to the contrastive loss for aligning the image and text modalities, a captioning loss is incorporated to predict image captions.
CONCH \cite{CONCH} and PRISM \cite{PRISM} both pre-train an image encoder on pathology datasets using the iBOT and DINOv2 frameworks, respectively, and then further conduct joint visual-language pre-training within the CoCa framework. The difference is that PRISM extends the image encoder to the WSI-level using a Perceiver network \cite{Perceiver} and employs WSIs along with their corresponding clinical reports for training.
Additionally, PathChat \cite{PathChat} is a pathology-focused MLLM, which uses UNI as the image encoder and further adopts a method similar to CONCH for vision-language pre-training. The trained image encoder is then connected to Llama 2 \cite{Llama2} and fine-tuned using various instructions.

Building upon prior work, TITAN \cite{TITAN} develops a multi-modal whole-slide foundation model primarily designed for training a slide encoder. Its pre-training process is divided into three stages. First, a slide encoder is trained using region crops under the iBOT framework with positional encoding incorporated. Subsequently, under the CoCa framework, the slide encoder is trained at both the tile-level and WSI-level, facilitating the gradual development of the model's ability to comprehend and generate meaningful vision-language representations for WSIs.



